Stability of Multi-Microgrids: New Certificates, Distributed Control, and Braess's Paradox

This paper investigates the theory of resilience and stability in multi-microgrid networks. We derive new sufficient conditions to guarantee small-signal stability of multi-microgrids in both lossless and lossy networks. The new stability certificate for lossy networks only requires local information, thus leads to a fully distributed control scheme. Moreover, we study the impact of network topology, interface parameters (virtual inertia and damping), and local measurements (voltage magnitude and reactive power) on the stability of the system. The proposed stability certificate suggests the existence of Braess's Paradox in the stability of multi-microgrids, i.e. adding more connections between microgrids could worsen the multi-microgrid system stability as a whole. We also extend the presented analysis to structure-preserving network models, and provide a stability certificate as a function of original network parameters, instead of the Kron reduced network parameters. We provide a detailed numerical study of the proposed certificate, the distributed control scheme, and a coordinated control approach with line switching. The simulation shows the effectiveness of the proposed stability conditions and control schemes in a four-microgrid network, IEEE 33-bus system, and several large-scale synthetic grids.

==> Section-3-Linearization_old.tex <==
\section{Linearization and Spectrum of Jacobian} \label{Sec: Linearization and Spectrum of Jacobian}
\subsection{Linearization}
Let us take the state variable vector $(\delta,\omega)\in\mathbb{R}^{2n}$ into account and note that the first step in studying the stability of multi-$\mu$G EPs is to analyze the Jacobian of the vector field in \eqref{eq: swing equations}: 
\begin{align}\label{eq: J}
J := \begin{bmatrix}
0 & I \\
-M^{-1} L  & - M^{-1}D \\
\end{bmatrix} \in\mathbb{R}^{2n\times 2n}
\end{align}
where $I\in\mathbb{R}^{n\times n}$ is the identity matrix, $M=   \mathbf{diag}(m_1,\cdots,m_n)$, and $D=\mathbf{diag}(d_1,\cdots,d_n)$. Throughout the paper, we assume $M$ and $D$ are nonsingular. Moreover, $L\in\mathbb{R}^{n\times n}$ is the Jacobian of the flow function with the entries:
\begin{subequations}\label{eq: Jacobian}
\begin{align} 
& L_{ii}= \sum \limits_{k=1, k \ne i}^n { V_i V_k Y_{ik} \sin \left( {\theta _{ik} - {\delta _i} + {\delta _k}} \right) }, \forall i \in \mathcal{N} \label{eq: Jacobian1}\\
&L_{ik}=  - {V_i} {V_k}{Y_{ik}}\sin \left( {{\theta _{ik}} - {\delta _i} + {\delta _k}} \right),\forall i\neq k \in \mathcal{N} \label{eq: Jacobian2}.
\end{align}
\end{subequations}
The matrix $L$ plays a prominent role in the spectrum of the Jacobian matrix $J$ (and as a consequence, in the stability properties of the EPs of multi-$\mu$Gs). We illustrate this role in the following subsection.

%
\subsection{Spectral Relationship Between Matrices $J$ and $L$}
%
We show that the eigenvalues of $J$ and $L$ are linked through a singularity constraint. Before proceeding to investigate this relationship, let us define the concept of matrix pencil \cite{2001-Tisseur-Pencil}. Consider $n\times n$ real matrices $Q_0,Q_1,$ and $Q_2$. A \emph{quadratic matrix pencil} is a matrix-valued function $P:\mathbb{C}\to\mathbb{R}^{n \times n}$ given by $\lambda \mapsto P(\lambda)$ such that  $P(\lambda) = \lambda^2Q_2 + \lambda Q_1 + Q_0$.
%
\begin{lemma} \label{lemma: relation between ev J and ev J11}
	$\lambda$ is an eigenvalue of $J$ if and only if the quadratic matrix pencil $P(\lambda):= \lambda^2 M + \lambda D + L$ is singular.
\end{lemma}
%
\begin{proof}
	Let $\lambda$ be an eigenvalue of $J$ and $(v_1 , v_2)$ be the corresponding eigenvector. Then	
	\begin{align} \label{eq: J cha eq}
	\begin{bmatrix}
	0 & I \\
	-M^{-1} L     &     - M^{-1}D \\
	\end{bmatrix}   \begin{bmatrix} v_1 \\v_2  \end{bmatrix}  = \lambda   \begin{bmatrix} v_1 \\v_2  \end{bmatrix}
	\end{align}
	which implies that $ v_2 = \lambda v_1$ and $(M^{-1} L + \lambda ( M^{-1} D  + \lambda I))v_1 = 0$, and consequently, 
	\begin{align}
	& \left(   \lambda^2 M + \lambda D + L \right) v_1 = 0. \label{eq: quadratic matrix pencil}
	\end{align}  
	Since the eigenvector $v$ is nonzero, we have $v_1 \not = 0$ (otherwise $v_2 = \lambda \times 0 = 0 \implies v = 0 $). Equation \eqref{eq: quadratic matrix pencil} implies that the matrix pencil $P(\lambda)= \lambda^2 M + \lambda D + L$ is singular.

	Conversely, 
	suppose there exists $\lambda \in \mathbb{C}$ such that $P(\lambda)= \lambda^2 M + \lambda D + L$ is singular. Choose a nonzero $v_1 \in   \mathbf{ker}(P(\lambda))$ and let $ v_2 := \lambda v_1$. 
	Accordingly, the characteristic equation \eqref{eq: J cha eq} holds, and consequently, $\lambda$ is an eigenvalue of $J$.
\end{proof}

Next, Proposition \ref{prop: geometric nullity of J and J11} illustrates the relationship between the kernels and the multiplicity of the zero eigenvalue of the two matrices $J$ and $L$.
%----------
\begin{proposition} \label{prop: geometric nullity of J and J11}
Consider the Jacobian matrix $J$ in \eqref{eq: J}. The following statements hold:
\begin{enumerate}[(i)]
    \item The kernel of $L$ is the orthogonal projection of the kernel of $J$ onto the linear subspace $\mathbb{R}^n \times \{0\}$. That is, $\mathbf{ker}(L)=  \mathbf{proj} (\mathbf{ker}(J))$. 
    
    \item  The geometric multiplicity of the zero eigenvalue in $\sigma(J)$ and $\sigma(L)$ are equal.
    
    \item $J$ is nonsingular if and only if $L$ is nonsingular.
\end{enumerate}
\end{proposition}
\begin{proof}
 See Appendix \ref{proof of prop: geometric nullity of J and J11}.
\end{proof}

As the role of $L$ in the spectrum of $J$ became more clear, we scrutinize the spectrum of $L$ in the next subsection. Our final goal is to use the spectral properties of $L$ together with the relationships established in Lemma \ref{lemma: relation between ev J and ev J11} and Proposition \ref{prop: geometric nullity of J and J11} to derive a stability certificate for multi-$\mu$Gs.

\subsection{Spectral Properties of $L$} \label{subsec: Spectral Properties of the Jacobian Matrix L}
% The Jacobian $L$ of the flow function \eqref{eq: flow function} is intertwined with the graph structure of the multi-$\mu$G network. To see this relation, let us define a weighted directed graph (digraph) $\mathcal{G}=(\mathcal{N},\mathcal{A},\mathcal{W})$ where each node $i\in\mathcal{N}$ corresponds to a microgrid and each directed arc $(i,k)\in\mathcal{A}$ corresponds to the entry $(i,k), i\ne k$ of the admittance matrix. We further define a weight for each arc $(i,k)\in\mathcal{A}$:
% \begin{align} \label{eq: weights of digraph lossy}
% w_{ik} = {V_i} {V_k}{Y_{ik}}\sin \left( \varphi_{ik} \right), 
% \end{align}
% where $\varphi_{ik} := {{\theta _{ik}} - {\delta _i} + {\delta _k}}$. With the above definition, we can see that each branch in the power network corresponds to two arcs of opposite direction in the digraph $\G$, while the arc weights depend on voltage angles and branch admittances. When $w_{ik}=0$, the branch $(i,j)$ is physically connected but electrically disconnected. We can also see that the Jacobian matrix $L$ of the flow function, which appeared in \eqref{eq: Jacobian}, is indeed the \emph{Laplacian} of the weighted digraph $\mathcal{G}$ defined as $L = D^+(\mathcal{G}) - A(\mathcal{G})$, where $D^+(\mathcal{G})$ is a diagonal matrix with the $i$-th diagonal entry being the sum of all the weights of the out-going arcs from node $i$, i.e., $D^{+}_{ii}(\mathcal{G})=\sum_{k=1, k\ne i}^n w_{ik}$. Moreover, $A(\mathcal{G})$ is the adjacency matrix of $\mathcal{G}$, i.e. $A_{ik}=w_{ik}$ and $0$ if there is no arc between $i$ and $k$.



Consider again the entries of $L$ spelled out in \eqref{eq: Jacobian}, and observe that $L_{ii}=\sum_{k=1, k\ne i}^n w_{ik}$ and $L_{ik}=-w_{ik}$ where 
\begin{align} \label{eq: weights of digraph lossy}
w_{ik} = {V_i} {V_k}{Y_{ik}}\sin \left( \varphi_{ik} \right), 
\end{align}
and $\varphi_{ik} = {{\theta _{ik}} - {\delta _i} + {\delta _k}}$. In general, the term $w_{ik}$ can be  positive, zero, or negative. In practice, however, if $Y_{ik}$ is non-zero (i.e., there exists a line connecting buses $i$ and $k$), $w_{ik}$ varies in a small positive range. Figure \ref{fig: histogram of angles} illustrates the histogram of the angle $\varphi_{ik}$ for all lines $(i,k)$ in different IEEE and NESTA standard distribution test cases, where the converged load flow data are obtained from \textsc{Matpower} \cite{matpower}. Accordingly, $\varphi_{ik} \in (0,\pi)$ in all of these cases. This observation stems from the fact that the entries of the admittance matrix, i.e., $Y_{ik} \measuredangle \theta_{ik}$ satisfy the following inequalities: $\theta_{ii} \in [ -\frac{\pi}{2} , 0 ), \: \forall i\in\mathcal{N}$ and $ \theta_{ik} \in [\frac{\pi}{2} , \pi), \: \forall (i,k)\in\mathcal{A}$ where the lower bounds are realized in lossless networks, and $\mathcal{A}$ denotes the set of lines in the distribution network.  
Thus, it is reasonable to assume that the EPs $(\delta^{*},\omega^{*})$ of the multi-$\mu$G dynamical system \eqref{eq: swing equations} are located in the set $\Omega$ defined as
\begin{align*}
\hspace{-2mm}\Omega = \left\{ (\delta,\omega)\in\mathbb{R}^{2n} :   0 < \theta_{ik}-\delta_i+\delta_k < \pi , \forall (i,k) \in \mathcal{A},\omega = 0  \right\}.
\end{align*}
%------------------------------------
\begin{figure}[t]
 \includegraphics*[width=3.5in, keepaspectratio=true]{figures//angle_assumption.pdf}
 \centering
  \caption{Histogram of the distribution of $\varphi_{ik}$ for all lines $(i,k)$ in different IEEE and NESTA standard test cases.}
  \label{fig: histogram of angles}
\end{figure}
Under this assumption, the terms $w_{ik} > 0$ for all lines $(i,k) \in \mathcal{A} $, and matrix $L$ turns out to be a \emph{singular $M$-matrix}. Recall that a matrix $A$ is an M-matrix if the off-diagonal elements of $A$ are non-positive and the non-zero eigenvalues of $A$ have positive real parts \cite{1974-M-matrices,1994-Berman-Nonnegative-matrices}.
\begin{proposition}\label{prop: quasi-M}
Let $(\delta^{*},\omega^{*})\in \Omega$ be an EP of the multi-$\mu$G system \eqref{eq: swing equations}. The Jacobian matrix $L$ defined by \eqref{eq: Jacobian} at this point has the following properties:
\begin{enumerate}[(i)]
	\item $L$ has a zero eigenvalue with an eigenvector $\mathbf{1}$, and the real part of each non-zero eigenvalue of $L$ is positive, i.e. $L$ is a singular $M$-matrix.
	
	\item If the distribution network has a connected underlying undirected graph, then the zero eigenvalue of $L$ is simple.
	%Both algebraic and geometric multiplicities of the zero eigenvalue of $L$ are  equal to the number connected components of .
		
	\item  $L =  \lambda_0 I - B$ for some nonnegative matrix $B$ (i.e., $b_{ij} \ge 0, \forall i, j$) and some $\lambda_0 \ge \rho$, where $\rho$ is the maximum eigenvalue of $B$.

	\item All principal minors of $L$ are non-negative.
	\end{enumerate}
%\textbf{I have to prove that an $L$ matrix which is weakly diagonally dominant is a quasi-M matrix }
% I need to prove that J11 is quasi-m matrix. Then I can use Theorem 3.1 of this paper.
%A Survey on M-Matrices
%Author(s): George Poole and Thomas Boullion
%Source: SIAM Review, Vol. 16, No. 4 (Oct., 1974), pp. 419-427
%Published by: Society for Industrial and Applied Mathematics
%Stable URL: https://www.jstor.org/stable/2028688
%Accessed: 29-10-2018 23:07 UTC
\end{proposition}

\begin{proof}
When $(\delta^{*},\omega^{*})\in \Omega$, we have 
$L_{ii} \ge 0$ for all $i\in\mathcal{N}$, and $L_{ik} \le 0, \: \forall (i,k), i \ne k$. Since $L$ has zero row sum, we have $L\mathbf{1}=0\implies0\in\sigma(L)$. Furthermore, the sum of the absolute values of the nondiagonal entries in the $i$-th row of $L$ is equal to $L_{ii}$, that is, $ L_{ii} = \sum_{k=1, k\ne i}^n |L_{ik}|$ for all $i\in \mathcal{N}$.
Let $\mathbb{D}(L_{ii})$ be a closed disc centered at $L_{ii}$ with radius $L_{ii}$. According to Ger\v{s}gorin circle theorem \cite{2013-Horn-matrix-analysis}, every eigenvalue of $L$ lies within at least one of the Ger\v{s}gorin discs $\mathbb{D}(L_{ii})$, which are located on the right half plane. This shows (i). 
The equivalence of (i) with (iii) and (iv) is a fundamental property of $M$-matrices \cite[Theorem 3.1]{1974-M-matrices},\cite[Theorem 4.6]{1994-Berman-Nonnegative-matrices}.
%-----------------------------------


To prove (ii), let us define a weighted directed graph (digraph) $\mathcal{G}=(\mathcal{N},\mathcal{A},\mathcal{W})$ where each node $i\in\mathcal{N}$ corresponds to a microgrid and each directed arc $(i,k)\in\mathcal{A}$ corresponds to the entry $(i,k), i\ne k$ of the admittance matrix. Moreover, let $w_{ik}$ defined in \eqref{eq: weights of digraph lossy} be the weight for each arc $(i,k)\in\mathcal{A}$. With the above definition, we can see that each branch in the power network corresponds to two arcs of opposite direction in the digraph $\G$, while the arc weights $w_{ik}$ are positive under the assumption $(\delta^{*},\omega^{*})\in \Omega$. Observe that the digraph $\G$ is strongly connected provided that the distribution network has a connected underlying undirected graph.

Accordingly, the Jacobian matrix $L$ of the flow function, is indeed the \emph{Laplacian} of the weighted digraph $\mathcal{G}$ defined as $L = D^+(\mathcal{G}) - A(\mathcal{G})$, where $D^+(\mathcal{G})$ is a diagonal matrix with the $i$-th diagonal entry being the sum of all the weights of the out-going arcs from node $i$, i.e., $D^{+}_{ii}(\mathcal{G})=\sum_{k=1, k\ne i}^n w_{ik}$. Moreover, $A(\mathcal{G})$ is the adjacency matrix of $\mathcal{G}$, i.e. $A_{ik}=w_{ik}$ and $0$ if there is no arc between $i$ and $k$. Now, we need the following lemma from graph theory to complete the proof: consider a weighted digraph $\mathcal{G}$ with positive weights and let $L$ be its Laplacian matrix. If $\mathcal{G}$ is strongly connected, then the zero eigenvalue of $L$ is simple \cite{2018-Bullo-book}. This completes the proof.
\end{proof}
%----------------------------------------
Properties (i) and (ii) of $L$ shown in the above proposition will be used in the next section to prove the main result of the paper. 
%
%The last missing information about the spectrum of $L$ is the exact algebraic multiplicity of the zero eigenvalue of $L$. Note that Proposition \ref{prop: quasi-M} asserts that this multiplicity is at least one. In the rest of this section, we will show that the multiplicity of the zero eigenvalue of $L$ is determined by the connectivity and weights of the digraph $\mathcal{G}$ induced by $L$. Let us first introduce the concept of a zero cut. Recall that a \textit{cut} $\mathcal{C}=(\mathcal{N}_1,\mathcal{N}_2)$ on graph ${\mathcal{G}}=(\mathcal{N},\mathcal{A})$ is a partition of the nodes $\mathcal{N}$ into two subsets $\mathcal{N}_1$ and $\mathcal{N}_2$ \cite{2018-Dorfler-algebraic-graph-theory}. The \textit{cutset} of a cut $\mathcal{C}=(\mathcal{N}_1,\mathcal{N}_2)$ is the set $\mathcal{A}(\mathcal{C})=\{(i,k) \in \mathcal{A} : i\in\mathcal{N}_1, k\in\mathcal{N}_2 \} \cup \{(i,k) \in \mathcal{A} : i\in\mathcal{N}_2, k\in\mathcal{N}_1 \}$ of arcs that have one endpoint in $\mathcal{N}_1$ and the other endpoint in $\mathcal{N}_2$.
%
% \begin{definition}
% A cut $\mathcal{C}_0$ is called a \textit{zero cut} if and only if $\left( {{\theta _{ik}} - {\delta _i} + {\delta _k}} \right) \in \{0,\pi\}$, i.e. $w_{ik}=0$, $\forall (i,k) \in  \mathcal{A}(\mathcal{C}_0)$.
% \end{definition}
%
%In other words, if $\mathcal{C}_0$ is a zero cut, then all the arcs in $\mathcal{A}(\mathcal{C}_0)$ have zero weight $w_{ik}=0$, which can be viewed as a certain electrical disconnectedness in the power network. Now we can determine the multiplicity of the zero eigenvalue of $L$ using the connectivity and zero cut of $\mathcal{G}$. Recall that a digraph $\Gamma$ is \emph{weakly connected} if the associated undirected graph, formed by removing all the directions of the arcs in $\Gamma$, is connected. Since each branch in the multi-$\mu$G system has two arcs in $\G$, hence, $\G$ is weakly connected if and only if the multi-$\mu$G system is connected.
%
% \begin{proposition} \label{prop: nullity of J11}
% Let $(\delta^{*},\omega^{*})\in \Omega$ be an EP of the multi-$\mu$G system \eqref{eq: swing equations}. The Jacobian matrix $L$ at this EP has exactly one zero eigenvalue if and only if the underlying directed graph $\mathcal{G}$ is weakly connected and has no zero cut.
% \end{proposition}
% \begin{proof}
% See Appendix \ref{app: proof of prop: nullity of J11}.
% \end{proof}

==> Section-4-Stability.tex <==
\section{Stability of Multi-Microgrid Networks} \label{Sec: Stability and Hyperbolicity of the Equilibrium Points}
Now we are ready to answer the fundamental question posed in Section \ref{subsec: Multi-Machine Swing Equations}: under what conditions is an EP $(\delta^*,\omega^*)$ locally asymptotically stable?
%
\subsection{The Main Stability Theorem}
\begin{theorem} \label{thm: stability properties}
    Let $(\delta^{*},\omega^{*})\in \Omega$ be an EP of the multi-$\mu$G system \eqref{eq: swing equations}. Let $B\in\mathbb{R}^{n\times n}$ denote the imaginary part of the admittance matrix. Suppose all microgrid interfaces have positive damping coefficient and inertia, and the linking grid $\G$ is connected. Then, the following statements hold:
    \begin{enumerate}[(a)]
        \item  The Jacobian $J$ at this EP has a zero eigenvalue with geometric multiplicity of one. \label{thrm-a}
        %with a one-dimensional invariant subspace $ \mathbf{span}(\mathbf{1})$.  
        \item All the nonzero real eigenvalues of $J$ are negative. \label{thrm-b}
        \item Let $Q_i$ be the net outgoing reactive power flow from microgrid PCC $i$. If 
        \begin{align} \label{eq: condition for stability}
            -Q_i - V_i^2 B_{ii} \le \frac{d_i^2}{2m_i}, &&    \forall i \in \mathcal{N} % \tag{\textbf{C}}
        \end{align}
        % $D_i^2-2M_iL_{ii}\ge0, \forall i \in \mathcal{N}$,
        then all the nonzero eigenvalues of $J$, both real and complex, are located in the left half plane, i.e., $\sigma(J)\subset\mathbb{C}_-\cup\{0\}$, and the EP is locally asymptotically stable. \label{thrm-c}
        
        \item If the transfer conductance of the lines is zero, then all the nonzero eigenvalues of $J$ are located in the left half plane, and the EP is locally asymptotically stable. \label{thrm-d}
         %and complex eigenvalues all with negative real parts.
    \end{enumerate}
\end{theorem}
%---------------
\begin{proof}
See Appendix \ref{app: proof of thm: stability properties}.
\end{proof}
\begin{remark}
Properties (\ref{thrm-a}) and (\ref{thrm-b}) hold independently of the sufficient conditions in (\ref{thrm-c}) and (\ref{thrm-d}). Property (\ref{thrm-d}) says if the network is lossless, then regardless of (\ref{thrm-c}), any EP is stable. If instead the network is lossy, then not every EP is stable and condition \eqref{eq: condition for stability} provides a new certificate to guarantee the small-signal stability of an EP. 
\end{remark}
\begin{remark}
    Notice that a salient feature of condition \eqref{eq: condition for stability} is that it only requires local information at each microgrid interface, hence, leads to a fully distributed control scheme to stabilize the multi-$\mu$G system. Detailed numerical simulation will be shown in Section \ref{Sec: Computational Experiments}.
\end{remark}
%----------------
% \begin{corollary} \label{coro: stability of EP set}
%     %Let $(\delta^{*},\omega^{*})\in \Omega$ be an EP of multi-$\mu$G system \eqref{eq: swing equations}. Suppose all microgrid interfaces have positive damping coefficient and inertia, and the underlying undirected graph of the system is connected.
%     Under the assumptions of Theorem \ref{thm: stability properties}, the set
%     \begin{align*}
%         \Gamma_{\delta^*}  = \left\{  (\delta ,\omega ) \in\mathbb{R}^{2n} : \delta = \delta^* + \alpha \mathbf{1},\forall \alpha \in \mathbb{R}, \omega = 0 \right\}
%     \end{align*}
%     is asymptotically stable if any of the following two conditions holds:
%     \begin{enumerate}
%      \item Condition \eqref{eq: condition for stability} holds.
%      \item The transfer conductance of the lines is zero.
%      \end{enumerate}
%     % The stable manifold of any equilibrium point is tangent to the hyperplane perpendicular to $\mathbf{1}$ and any point along $ \mathbf{span} (\mathbf{1})$ is an equilibrium point.
% \end{corollary}
%---------------------------
% \begin{remark}
%     The simple zero eigenvalue of the Jacobian matrix $J$ (and the resultant center manifold) stems from the translational invariance of the flow function \eqref{eq: flow function}. As we mentioned in Section \ref{subsec: Multi-Machine Swing Equations}, we can eliminate this eigenvalue by choosing a reference bus and refer all other bus angles to it. Therefore, the set of EPs $\Gamma_{\delta^*}$ will collapse into one EP. Such an EP will be hyperbolic and asymptotically stable under the conditions of Corollary \ref{coro: stability of EP set}.
% \end{remark}
%
%
\subsection{Intuition and Paradox Behind Condition \eqref{eq: condition for stability}}

Condition \eqref{eq: condition for stability} in Theorem \ref{thm: stability properties} provides a practical and efficient way to certify the stability of the EPs in general lossy multi-$\mu$G networks. It also introduces a distributed control rule for tuning the interface parameters of each microgrid without compromising the network stability.
%Moreover, it can be incorporated into the multi-$\mu$G scheduling problem as an additional constraint, thereby guaranteeing the transient stability of the solution. 
In this section, we will explore the intuition behind this theory as well as two interesting paradoxes that come with it.

%\begin{remark} \hfill
    \begin{itemize}

    \item \emph{\textbf{Note 1:}}
    The variable $Q_i$ in \eqref{eq: condition for stability} is the net reactive power that microgrid $i$ injects into the rest of the multi-$\mu$G network, that is, if microgrid $i$ is supplying reactive power, then $Q_i>0$. Otherwise, if it is consuming reactive power, then $Q_i<0$. Intuitively, when microgrid $i$ is a supplier of reactive power, the first term on the left-hand side of \eqref{eq: condition for stability} is negative, and this situation will help condition \eqref{eq: condition for stability} hold. 
    
    \item
    \emph{\textbf{Note 2:}} 
    Recall that $Y_{ii}\measuredangle \theta_{ii}=G_{ii}+jB_{ii} = \sum_{k=1}^n y_{ik}$, where $y_{ik}=g_{ik}+jb_{ik}$ is the admittance of line $(i,k)$, with $g_{ik}\ge0$ and $b_{ik}\le0$. Therefore, $B_{ii}\le0$, and the second term on the left-hand side of \eqref{eq: condition for stability} is always positive. Here, it is assumed that $y_{ii}$, i.e., the admittance-to-ground at PCC $i$ is negligible. Otherwise, we may have $B_{ii}>0$, and the second term on the left-hand side of \eqref{eq: condition for stability} could be negative.
    
    \item
    \emph{\textbf{Note 3:}}
    The first two notes clarify that the left-hand side of \eqref{eq: condition for stability} can be negative if microgrid $i$ is supplying reactive power; otherwise it is positive. Consequently, condition \eqref{eq: condition for stability} is not trivial.
    
    \item
    \emph{\textbf{Note 4:}}
    Condition \eqref{eq: condition for stability} enforces an upper bound which is proportional to the square of damping and inverse of inertia. This is consistent with the intuition that if we increase the damping, the stability margin of the system will increase. However, it is not intuitive (could be a paradox) that decreasing the virtual inertia of a microgrid interface will increase the stability margin.
    
    \item
    \emph{\textbf{Note 5:}} By adding more transmission lines to the system, $|B_{ii}|$ will increase, and this in turn could increase the left-hand side of \eqref{eq: condition for stability} and lead to the violation of this condition. This can be called the Braess's Paradox in power system stability.
    %
    %which reveals that adding a road to a particular congested traffic network would increase overall journey time.
    \end{itemize}
%\end{remark}
The following corollary will further illustrate the aforementioned Braess's Paradox.
\begin{corollary} \label{coro: paradox}
Under the assumptions of Theorem \ref{thm: stability properties}, if 
\begin{align} \label{eq: condition for stability without sin}
            \sum \limits_{k=1, k \ne i}^n { V_i V_k Y_{ik} } \le \frac{d_i^2}{2m_i},     && \forall i \in \mathcal{N}
            %\tag{\textbf{C-1}}
\end{align}
then the nonzero eigenvalues of $J$ are located in the left half plane and the EP is locally asymptotically stable.%i.e., $\sigma(J)\subset\mathbb{C}_-\cup\{0\}$.
\end{corollary}
%Recall that $Y_{ik}\measuredangle \theta_{ik} = - y_{ik}$, i.e., it is the negative of the admittance between the nodes $i$ and $j$.


This corollary directly follows from the proof of Theorem \ref{thm: stability properties} provided in Appendix \ref{app: proof of thm: stability properties}. Counterintuitively, according to \eqref{eq: condition for stability without sin}, adding more power lines can lead to violating the sufficient condition for stability. This Braess's Paradox in power systems has been also acknowledged in \cite{2015-robustness-paradox-network} and \cite{Vu-2019-reconfig-microgrids} in different contexts and using different approaches. 
%
\textcolor{blue}{
Note that removing lines from a network could make the system more vulnerable to contingencies and eliminate the reliability benefits of having more transmission line capacity. This trade-off should be taken into account during the design and operation of power grids. 
}



%------------------------------------------------------------------------

%\subsection{Structure-Preserving Higher-Order Microgrids}
\subsection{Stability Condition in Structure-Preserving Networks}
\label{subsec: structure-preserving microgrid}
%
%\section{Understanding The effect of Kron Reduction}
%
\textcolor{blue}{
As discussed in Section \ref{subsec: Multi-Machine Swing Equations},
each node in the linking grid $\mathcal{G}=(\mathcal{N},\mathcal{E})$ represents a microgrid, which is modeled by a second-order ODE in \eqref{eq: swing equations}. 
In this section, we study how the internal structure of microgrids can be incorporated into model \eqref{eq: swing equations}, allowing higher order models for each microgrid,
and then we find a transformation of the stability condition \eqref{eq: condition for stability} in such structure-preserving networks.
%
%$\mathcal{G}=(\mathcal{N},\mathcal{E})$, where $\mathcal{N}$ is the set of nodes and $\mathcal{E}$ is the set of edges. Each node in $\mathcal{N}$ represents a microgrid and each edge in $\mathcal{E}$ represents an electrical branch connecting the two microgrids across the branch. We will refer to $\mathcal{G}$ as the linking grid
%
Let $\mathcal{G}_i = (\mathcal{N}_i, \mathcal{E}_i)$ denote the internal power grid associated with microgrid $i\in\mathcal{N}$. 
Moreover suppose $\mathcal{G}^d = (\mathcal{N}^d, \mathcal{E}^d)$ is the distribution network including the subgraphs $\mathcal{G}_i$ associated with each microgrid $i\in\mathcal{N}$.
%
Observe that the linking grid $\mathcal{G}$ corresponding to the multi-$\mu$G $\mathcal{G}^d$ is indeed the condensation of $\mathcal{G}^d$, that is, each node of $\mathcal{G}$ is a super node that represents a microgrid.
%
% defined as follows: the nodes of 
%condensation graph of $\mathcal{G}$ is 
%
%: the entire distribution network including the linking grid $\mathcal{G} = (\mathcal{N}, \mathcal{E})$ and 
%
%Note that
%
%For each $i\in\mathcal{N}$, the internal grid $\mathcal{G}_i$ is connected to node $i\in\mathcal{N}$ of the linking grid.
%
%Let $\mathscr{G}$ represent the expanded multi-microgrid network including the linking grid $\mathcal{G} = (\mathcal{N}, \mathcal{E})$, where each node $i\in\mathcal{N}$ is connected to a microgrid with graph $\mathcal{G}_i$.
%
%the linking grid $\mathcal{G}$ through
%undirected graph associated with this microgrid. 
%Each node in $\mathcal{N}_i$ represents an interior nodes of microgrid $i$
%Let interior topology of microgrid 
%Let $\alpha$ denote the set of interior nodes of microgrid $i\in\mathcal{N}$.
The set of nodes $\mathcal{N}_i$ may include active nodes (i.e., those connected to DGs and/or VSIs) as well as passive nodes (i.e., those connected to a load). 
%Assuming that the loads in each microgrid are modeled as constant admittances, 
Now, each microgrid $\mathcal{G}_i$ can be Kron reduced to network  $\mathcal{G}_i^r$ consisting of only active nodes, defined as follows:
%
% the loads
% are modeled as constant current injections
%
%
%We assume each microgrid is connected to the linking grid through
%
% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.3\linewidth]{Kron.jpg}
% 	\caption{Topological evolution of the multi-microgrid network following the reduction of microrgid internal network.}
% 	\label{fig: Kron reduction}
% \end{figure}
%Before conducting stability analysis, 
%In the sequel, 
%for $A\in\mathbb{C}^{n\times n}$ and $\alpha,\beta \subseteq\{1,...,n\}$, the submatrix of entries that lie in the rows indexed by $\alpha$ and and
% columns indexed by $\beta$ is denoted by $A[\alpha, \beta]$. Similarly, for a vector $x\in\mathbb{C}^{n}$, $x[\alpha]$ denotes the subvector consisting of entries indexed by $\alpha$
%
\begin{definition} \label{def: Kron}
	Let $Y$ be the nodal admittance matrix of the microgrid $\mathcal{G}_i = (\mathcal{N}_i, \mathcal{E}_i)$ where the set of active and passive nodes are denoted by $\alpha,\beta \subseteq\mathcal{N}_i$, respectively. The Kron reduction or Schur complement of $Y$ with respect to the block $Y[\beta,\beta]$ is the $|\alpha|\times|\alpha|$ matrix $Y^{r} = Y[\alpha,\alpha] - Y[\alpha,\beta] Y[\beta,\beta]^{-1} Y[\beta,\alpha]$. The graph induced by $Y^r$ is denoted by $\mathcal{G}_i^r$.
\end{definition}
%
Recall that in small-signal stability studies, loads are considered constant admittances and reflected into the diagonal entries of the nodal admittance matrix $Y$. This inclusion of loads transforms the matrix $Y\in\mathbb{C}^{n\times n}$ from a Laplacian matrix to a loopy Laplacian matrix which has a nonzero row sum and induces a graph with self loops. This loopy Laplacian matrix can be better studied by introducing an additional \emph{ground node} and defining an augmented nodal admittance matrix where loads are connected to the ground node instead of being modeled as self-admittances. Such an augmented nodal admittance matrix has a zero row sum. Interestingly, this ground node augmentation and Kron reduction commute \cite{2012-dorfler-kron}, i.e., the order of these two transformations can change and they lead to the same result. Based on this property and without loss of generality, we assume the ground node augmentation is already performed and therefore the nodal admittance matrix has zero row sum. Now, let us define the following assumptions:
%
\begin{assumption} \label{as: y_matrix sign}
The nodal admittance matrix $Y=G+jB$ satisfies $G_{ik}\le0, B_{ik}\ge0,$ for all $i\ne k$, and $G_{ii}\ge0, B_{ii}\le0$ for self-admittances. 
%
%2) There exist real numbers $\nu_{\min}$ and $\nu_{\max}$ such that $ \sqrt{ (\nu_{\max}^2-1)/2}  \le \nu_{\min} \le \nu_{\max}$ and   
%$\nu_{\min} |G_{ik}| \le |B_{ik}| \le \nu_{\max} |G_{ik}| $, for all $i,k$.
%
%2) There exist real numbers $\nu_{\min}$ and $\nu_{\max}$ such that $\nu_{\min} \le \nu_{\max}$, $\nu_{\min}^3 + 2\nu_{\min} - \nu_{\max} \ge 0$, and   
%$\nu_{\min} |B_{ik}| \le |G_{ik}| \le \nu_{\max} |B_{ik}| $, for all $i,k$.
%
%$\nu |G_{ik}| =  |B_{ik}| $, for all $i,k$.
%2) There exists a real number $\nu > 1$ such that $\nu |G_{ik}| =  |B_{ik}| $, for all $i,k$.
\end{assumption}
%
%
\begin{assumption} \label{as: y_matrix bound}
%1) The nodal admittance matrix $Y=G+jB$ satisfies $G_{ik}\le0, B_{ik}\ge0,$ for all $i\ne k$, and $G_{ii}\ge0, B_{ii}\le0$ for self-admittances. 
%
Let $Y=G+jB$ be the nodal admittance matrix. 
There exist real numbers $\nu_{\min}$ and $\nu_{\max}$ such that $ \sqrt{ (\nu_{\max}^2-1)/2}  \le \nu_{\min} \le \nu_{\max}$ and   
$\nu_{\min} |G_{ik}| \le |B_{ik}| \le \nu_{\max} |G_{ik}| $, for all $i,k$.
%
%2) There exist real numbers $\nu_{\min}$ and $\nu_{\max}$ such that $\nu_{\min} \le \nu_{\max}$, $\nu_{\min}^3 + 2\nu_{\min} - \nu_{\max} \ge 0$, and   
%$\nu_{\min} |B_{ik}| \le |G_{ik}| \le \nu_{\max} |B_{ik}| $, for all $i,k$.
%
%$\nu |G_{ik}| =  |B_{ik}| $, for all $i,k$.
%2) There exists a real number $\nu > 1$ such that $\nu |G_{ik}| =  |B_{ik}| $, for all $i,k$.
\end{assumption}
%
Before proceeding to the main result of this section,
let us present the following useful lemmas.
%
\begin{lemma} \label{lem: schur-complement-close}
    The following two classes of matrices are invariant under Kron reduction: i) matrices with zero row sum; ii) symmetric matrices. In other words, zero row summation and symmetry of matrices remain unchanged after Kron reduction.
\end{lemma}
%
% \begin{proof}
%     Let $Y\in\mathbb{C}^{n\times n}$ have zero row sum, i.e., $Y\mathbf{1}_n = 0$, where $\mathbf{1}_n\in\mathbb{R}^n$ is the vector of all ones. With $\alpha = \{1,\cdots, n-|\beta|\}$ and $\beta = \{n-|\beta|+1,\cdots, n\}$, we have 
%     \begin{align*}
%         \begin{bmatrix}
%         Y[\alpha,\alpha] & Y[\alpha, \beta] \\
%         Y[\beta, \alpha] & Y[\beta, \beta]
%         \end{bmatrix}
%         %
%         \begin{bmatrix}
%         \mathbf{1}_{|\alpha|} \\ \mathbf{1}_{|\beta|}
%         \end{bmatrix}
%         = 0.
%     \end{align*}
%     The row sum of the Schur complement $Y^{r} \in \mathbb{C}^{|\alpha| \times |\alpha|}$ is 
%     \begin{align*}
%     	Y^{r} \mathbf{1}_{|\alpha|} &= Y[\alpha,\alpha] \mathbf{1}_{|\alpha|} - Y[\alpha,\beta] Y[\beta,\beta]^{-1} Y[\beta,\alpha] \mathbf{1}_{|\alpha|} \\
%     	&= Y[\alpha,\alpha] \mathbf{1}_{|\alpha|} + Y[\alpha,\beta] Y[\beta,\beta]^{-1} Y[\beta,\beta] \mathbf{1}_{|\beta|} \\
%     	&= Y[\alpha,\alpha] \mathbf{1}_{|\alpha|} +
%     	Y[\alpha,\beta] \mathbf{1}_{|\beta|} = 0.
%     \end{align*}
%       This proves the first part of the lemma.
%       The class of symmetric matrices $Y=Y^\top$ is also closed under Schur complementation, because
%       \begin{align*}
%     	{Y^{r}}^\top &= Y[\alpha,\alpha]^\top - Y[\beta,\alpha]^\top  Y[\beta,\beta]^{-\top} Y[\alpha,\beta]^\top \\
%     	&= Y[\alpha,\alpha] - Y[\alpha,\beta] Y[\beta,\beta]^{-1} Y[\beta,\alpha] = Y^r,
%     \end{align*}
%     where the last equality holds because the symmetry of $Y$ implies that $Y[\alpha,\alpha]^\top = Y[\alpha,\alpha]$, $Y[\beta,\alpha]^\top = Y[\alpha, \beta]$, and  $Y[\beta,\beta]^{-\top} = Y[\beta,\beta]^{-1}$. 
% \end{proof}
%----------------------------
%---------------------------
%
\begin{lemma} \label{lem: assumption closed Kron}
    Let $\mathcal{Y}$ and $\mathcal{Y}'$ be the classes of nodal admittance matrices that satisfy Assumptions \ref{as: y_matrix sign} and \ref{as: y_matrix bound}, respectively. Suppose $\mathcal{Y}'$ is invariant under Kron reduction, i.e., any admittance matrix $Y$ that satisfies Assumption \ref{as: y_matrix bound} will still satisfy this assumption after Kron reduction. 
    Then $\mathcal{Y}\cap\mathcal{Y}'$ is also invariant under Kron reduction.
\end{lemma}
%
%---------------------------
%
%See Appendix \ref{sec: proof of lem: assumption closed Kron lossless}
%
% \begin{lemma} \label{lem: assumption closed Kron lossless}
%     Let $\mathcal{Y}$ be the class of lossless nodal admittance matrices that satisfy Assumption \ref{as: y_matrix sign}.
%     Then $\mathcal{Y}$ is closed under Kron reduction.
% \end{lemma}
%
The proof of Lemma \ref{lem: schur-complement-close} can be found for example in \cite{2012-dorfler-kron}, and Lemma \ref{lem: assumption closed Kron} is proved in Appendix \ref{sec: proof of lem: assumption closed Kron}.
%and Lemma \ref{lem: assumption closed Kron lossless} can be proved similarly.
%
% \textcolor{purple}{
% \begin{proof}
%     %Let us first prove that the class of matrices with zero row sum is closed under Schur complementation. 
% According to Lemma \ref{lem: schur-complement-close}, the Kron reduction of an admittance matrix $Y$ is again a symmetric matrix with zero row sum, and therefore corresponds to a well-defined reduced network.    
% Let the distribution network $\mathcal{G} = (\mathcal{N}, \mathcal{E})$ have the nodal admittance matrix $Y\in\mathbb{C}^{n \times n}$. The purpose of Kron reduction here is to remove the set of passive nodes of microgrid $\mu$ denoted by $\beta = \mathcal{N}_\mu \setminus \alpha$.
% %
% After properly labeling the nodes, we can have $\beta = \{n-|\beta| + 1, \cdots , n\}$.
% The Kron reduction of nodes in $\beta$
% can be accomplished by constructing a sequence of matrices $\{Y^{(\ell)}\}_{\ell =1}^{|\beta|}$, where $Y^{(\ell)}\in\mathbb{C}^{(n-\ell)\times(n-\ell)}$ is defined as
% \begin{align}
% 	Y^{(\ell)}_{ik} = Y^{{(\ell-1)}}_{ik} - {Y^{(\ell-1)}_{im_\ell}Y^{(\ell-1)}_{m_\ell k}} /{Y^{(\ell-1)}_{m_\ell m_\ell}}, && i, k \in\{ 1, \cdots, n-\ell \}
% \end{align}
% where $Y^{(0)} = Y$, $Y^{(|\beta|)} = Y^{r}$, and $m_\ell = n - \ell +1$. The matrix sequence $\{Y^{(\ell)}\}_{\ell =1}^{|\beta|}$ is well-defined, and according to Lemma \ref{lem: schur-complement-close}, each $Y^{(\ell)}$ is a nodal admittance matrix of a well-defined network.
% %
% %
% Consider $Y_{ik}^{(\ell - 1)} = G_{ik} + j B_{ik}$ and note that
% we have dropped the superscript $(\ell-1)$ on $G_{ik}$ and $B_{ik}$ for notational simplicity.
% Let us focus on the off-diagonal entries $Y^{(\ell)}_{ik}, i\ne k$. 
% % \begin{align}
% % 	Y^{(\ell)}_{ik} &= Y^{{(\ell-1)}}_{ik} - {Y^{(\ell-1)}_{im_\ell}Y^{(\ell-1)}_{m_\ell k}} /{Y^{(\ell-1)}_{m_\ell m_\ell}} \\
% % 	&= G_{ik} + j B_{ik} - (G_{im_\ell} + j B_{im_\ell})(G_{m_\ell k} + j B_{m_\ell k}) / (G_{m_\ell m_\ell } + j B_{m_\ell m_\ell}) \\
% % 	& = G_{ik} + j B_{ik} - 
% % 	(	(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% % 	+j(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k})	) / (G_{m_\ell m_\ell } + j B_{m_\ell m_\ell})\\
% % 	%
% % 	& = G_{ik} + j B_{ik} - 
% % 	(	(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% % 	+j(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k})	) (G_{m_\ell m_\ell } - j B_{m_\ell m_\ell}) / (G_{m_\ell m_\ell }^2 +  B_{m_\ell m_\ell}^2) \\
% % 	%
% % 	%
% % 	& = G_{m_\ell m_\ell }(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% % 	+B_{m_\ell m_\ell}(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k}) \\
% % 	%
% % 	&+j(
% % 	G_{m_\ell m_\ell }(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k})
% % 	-B_{m_\ell m_\ell}(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% % 	)
% % 	%
% % \end{align}
% \begin{align}
% 	Y^{{(\ell-1)}}_{ik} - Y^{(\ell)}_{ik} &=   {Y^{(\ell-1)}_{im_\ell}Y^{(\ell-1)}_{m_\ell k}} /{Y^{(\ell-1)}_{m_\ell m_\ell}} \\
% 	&=  (G_{im_\ell} + j B_{im_\ell})(G_{m_\ell k} + j B_{m_\ell k}) / (G_{m_\ell m_\ell } + j B_{m_\ell m_\ell}) \\
% 	& = 
% 	(	(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% 	+j(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k})	) / (G_{m_\ell m_\ell } + j B_{m_\ell m_\ell})\\
% 	%
% 	& =  
% 	(	(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% 	+j(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k})	) (G_{m_\ell m_\ell } - j B_{m_\ell m_\ell}) /\eta \\
% 	%
% 	%
% 	& =( G_{m_\ell m_\ell }(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% 	+B_{m_\ell m_\ell}(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k}) )/\eta \\
% 	%
% 	& +j(
% 	G_{m_\ell m_\ell }(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k})
% 	-B_{m_\ell m_\ell}(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% 	)/\eta
% 	%
% \end{align}
% where $\eta = G_{m_\ell m_\ell }^2 +  B_{m_\ell m_\ell}^2$. 
% Observe that
% \begin{align}
% \Im({Y^{(\ell-1)}_{im_\ell}Y^{(\ell-1)}_{m_\ell k}} /{Y^{(\ell-1)}_{m_\ell m_\ell}}) \eta &= 
%     G_{m_\ell m_\ell }G_{im_\ell}B_{m_\ell k} + G_{m_\ell m_\ell }B_{im_\ell}G_{m_\ell k} \\
% 	&-B_{m_\ell m_\ell}(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k}) \le 0,
% \end{align}
% Because under Assumption \ref{as: y_matrix}, we have
% \begin{align*}
%   G_{m_\ell m_\ell }G_{im_\ell}B_{m_\ell k} \le 0,
%   G_{m_\ell m_\ell }B_{im_\ell}G_{m_\ell k} \le 0,
%   G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k} \le 0,
%   -B_{m_\ell m_\ell} >0. 
% \end{align*}
% Also note that
% \begin{align}
%   \Re({Y^{(\ell-1)}_{im_\ell}Y^{(\ell-1)}_{m_\ell k}} /{Y^{(\ell-1)}_{m_\ell m_\ell}}) \eta &=  G_{m_\ell m_\ell }(G_{im_\ell}G_{m_\ell k} - B_{im_\ell}B_{m_\ell k})
% 	+B_{m_\ell m_\ell}(G_{im_\ell}B_{m_\ell k} + B_{im_\ell}G_{m_\ell k}) \\
% 	&= G_{m_\ell m_\ell}G_{im_\ell}G_{m_\ell k} - G_{m_\ell m_\ell}B_{im_\ell}B_{m_\ell k}
% 	+B_{m_\ell m_\ell}G_{im_\ell}B_{m_\ell k} + B_{m_\ell m_\ell}B_{im_\ell}G_{m_\ell k}\\
% 	%
% 	&= G_{m_\ell m_\ell}G_{im_\ell}G_{m_\ell k} - \nu^2 G_{m_\ell m_\ell} G_{im_\ell} G_{m_\ell k} 
% 	+\nu^2 G_{m_\ell m_\ell}G_{im_\ell}G_{m_\ell k} + \nu^2 G_{m_\ell m_\ell}G_{im_\ell}G_{m_\ell k} \\
% 	&= (1+\nu^2)G_{m_\ell m_\ell}G_{im_\ell}G_{m_\ell k} \ge 0
% \end{align}
% Consider the following two cases for all $i\ne k$:
% \begin{enumerate}
%     \item If $i$ is connected to $k$ in the graph $\mathcal{G}^{(\ell-1)}$, i.e.,     $Y^{{(\ell-1)}}_{ik}$ is nonzero with $\Re(Y^{{(\ell-1)}}_{ik}) \le0$, $\Im(Y^{{(\ell-1)}}_{ik}) > 0$, then $Y^{{(\ell)}}_{ik}$ is also nonzero with $\Re(Y^{{(\ell)}}_{ik}) \le0$, $\Im(Y^{{(\ell)}}_{ik}) > 0$.
%     %\item If $Y^{{(\ell-1)}}_{ik} = 0$ , then $Y^{{(\ell)}}_{ik}$ is also nonzero with $\Re(Y^{{(\ell)}}_{ik}) \le0$, $\Im(Y^{{(\ell)}}_{ik}) > 0$.
%     %
%     \item If there is a path from $i$ to $k$ in $\mathcal{G}^{(\ell-1)}$ whose nodes are $\{i,k,m_{\ell}\}$, then $Y^{{(\ell)}}_{ik}$ is also nonzero with $\Re(Y^{{(\ell)}}_{ik}) \le0$, $\Im(Y^{{(\ell)}}_{ik}) > 0$.
% \end{enumerate}
% %
% According to the above rule, the entry $Y_{ik}^r$ of the Kron reduced matrix is nonzero if and only if there is a path from $i$ to $k$ that includes ${i,k}$ or the passive nodes $\beta$.
% \end{proof}
% }
%--------------------------------------------------
%\subsubsection{Transforming the Certificate to the Structure-Preserving Network}
%--------------------
% It is known that
% Moreover, the following lemma formalizes a well-known fact from o
%------------------------------------
% \begin{lemma} \label{lem: power in Kron reduction}
% 	Consider an $n$-bus power system with the vector of nodal voltages $V\in\mathbb{C}^n$ and power injections $S\in\mathbb{C}^n$.
% 	Let $\alpha\subset\{1,...,n\}$ denote the set of active nodes. 
% 	If the vector of nodal voltages of the reduced network is $V[\alpha]$, then the vector of power injections in the reduced network is $S[\alpha]$.
% \end{lemma}
%
% See Appendix \ref{sec: proof of lem: power in Kron reduction}
%--------------------------------------
% \begin{remark}
% Consider the reduced swing equation model
% \begin{align} \label{eq: reduced swing equations}
% M \ddot \delta  + D \dot \delta = P_m^r - P^r_e(\delta(t)),
% \end{align}
% where $\delta\in\mathbb{R}^{|\alpha|}$, $M,D\in\mathbb{R}^{|\alpha|\times |\alpha|}$, $P_m^{r} \in \mathbb{R}^{|\alpha|}$. 
% Moreover, $P^{r}_e(\delta(t)): \mathbb{R}^{|\alpha|} \to \mathbb{R}^{|\alpha|}$ is the vector of real power injections in the reduced network.
% %
% %\begin{subequations} \label{eq: reduced swing equations}
% %	\begin{align}
% %	& \dot{\delta}_i(t) = \omega_i(t) && \forall i \in {\alpha},  \label{eq: reduced swing equations a}\\
% %	& m_i \dot{\omega}_i(t)+ d_i \omega_i(t) = P_{s_i} - P_{e_i}(\delta(t)) && \forall i \in \alpha, \label{eq: reduced swing equations b}
% %	\end{align}
% %\end{subequations}
% %
% The structure-preserving counterpart of the above model is
% \begin{align} \label{eq: st preserving swing equations}
% M \ddot \delta  + D \dot \delta &= P_m[\alpha] - P_e(\delta(t), \delta^\ell(t))[\alpha], \\
% 0 &= P_m[\beta] - P_e(\delta(t), \delta^\ell(t))[\beta],
% \end{align}
% where $\delta^\ell\in\mathbb{R}^{|\beta|}$ is the vector of voltage angles at passive nodes. Note that $P_m[\alpha] = P_m^r$ is the vector of mechanical powers at active nodes, and $P_m[\beta]$ is the vector of active power consumption at passive nodes. 
% Observe that the structure-preserving swing equation model is indeed a system of differential algebraic equations contrary to the reduced model that is a system of ordinary differential equations. %
% Now, according to Lemma \ref{lem: power in Kron reduction}, if at any time $t\ge0$ the voltage magnitudes are fixed and equal in the two models (which is a reasonable assumption in small-signal stability studies), we have $P^r_e(\delta(t)) = P_e(\delta(t), \delta^\ell(t))[\alpha]$.
% %
% %The above lemma shows if the voltage magnitudes is fixed and equal in the two models (which is a reasonable assumption in small-signal stability studies), then the active power injection vector in the reduced network $P_{r}$ is equal to the subvector $P[\alpha]$ in the original network. 
% As a consequence, if the reduced swing equation model and its structure-preserving counterpart start from the same initial condition, their trajectories $\{(\delta(t),\dot\delta(t)): t\ge 0\}$  will be the same.
% %the dynamical model governing the 
% \end{remark}
%-----------------
Recall that condition \eqref{eq: condition for stability} in Theorem \ref{thm: stability properties} is derived for the linking grid $\mathcal{G}=(\mathcal{N},\mathcal{E})$ where all nodes are active, i.e., each microgrid is represented by $\mathcal{G}_i = (\mathcal{N}_i, \mathcal{E}_i)$ with $|\mathcal{N}_i|=1$ and $\mathcal{E}_i=\emptyset$. 
%
The next theorem revisits this stability condition for more general cases such that each microgrid $\mathcal{G}_i = (\mathcal{N}_i, \mathcal{E}_i)$ may include an arbitrary combination of both active and passive nodes. 
%
%
%the Kron-reduced network. The next Theorem clarifies the transformation of the stability criterion in the original network.
%shows that under reasonable assumptions, condition (12) can be converted to a stability criterion in the original network.
\begin{theorem} \label{thrm: stability of original net}
Let $\alpha_i$ be the set of active nodes in microgrid $i\in\mathcal{N}$.
The following statements hold:
\begin{enumerate}[(a)]
    \item If 
        \begin{align} \label{eq: stability condition orig net Br}
    		-Q_k - V_k^2 B_{kk}^r \le \frac{d_k^2}{2m_k} && \forall k\in\alpha_i, i \in \mathcal{N},
    	\end{align}
    	then the EP is locally asymptotically stable. Here $B_{kk}^r$ is the $k$th diagonal entry of the imaginary part of the reduced admittance matrix.
    \label{thrm: stability of original net - a}	
    \item Suppose Assumption \ref{as: y_matrix sign} holds for network    $\mathcal{G}^d$, and its reduced nodal admittance matrix with   respect to subsets of passive nodes             $\mathcal{N}^d \setminus \{\cup_i\alpha_i\} $ satisfies Assumption \ref{as: y_matrix bound}. If
       \begin{align} \label{eq: stability condition orig net B}
    		-Q_k - V_k^2 B_{kk} \le \frac{d_k^2}{2m_k} && \forall k\in\alpha_i, i \in \mathcal{N}
    	\end{align}
    then the EP is locally asymptotically stable.
    \label{thrm: stability of original net - b}
\end{enumerate}
%
% 	Under Assumption \ref{as: y_matrix}, if
% 	\begin{align} \label{eq: stability condition orig net}
% 		-Q_i - V_i^2 B_{ii} \le \frac{d_i^2}{2m_i} && \forall i \in \mathcal{N}\setminus \beta
% 	\end{align}
% holds, then condition (12) in Theorem 1 holds for the Kron-reduced network. Note that	in \eqref{eq: stability condition orig net}, the quantities $Q_i, V_i, B_{ii}, d_i, m_i$ correspond to the original network.
\end{theorem}
The proof of this theorem is given in
Appendix \ref{sec: proof of thrm: stability of original net}.
Notice that in \eqref{eq: stability condition orig net B}, $B_{kk}$ is the $k$th diagonal entry of the imaginary part of the original admittance matrix, as opposed to the term $B_{kk}^r$ in \eqref{eq: stability condition orig net Br} which corresponds to the Kron reduced network. In comparison with \eqref{eq: stability condition orig net Br}, condition \eqref{eq: stability condition orig net B} is more conservative and needs additional assumption; however, it is suitable for applications where keeping the topology of the original network is necessary, e.g., studying the role of network topology on the system stability.
}
%
%-----------------------------------------------------------
%-----------------------------------------------------------
%---------------------------
% \subsubsection{Topological effects of Kron reduction on Microgrid PCCs}

% The next proposition describes the topological properties of the linking graph, under the Kron reduction of microgrids.
% Here, we also consider the possibility that microgrid $\mathcal{G}_i$ is connected to the rest of the grid through multiple PCCs. 

% \begin{proposition}[Topological effects of Kron reduction] \label{prop: effects of Kron reduction}
% Consider a microgrid $\mathcal{G}_{\mu} = (\mathcal{N}_{\mu}, \mathcal{E}_{\mu})$ which is part of a larger distribution network
% $\mathcal{G} = (\mathcal{N}, \mathcal{E})$.
% %
% Suppose $\alpha \subseteq \mathcal{N}_{\mu}$ is the set of active nodes of microgrid ${\mu}$.
% Moreover, let $\gamma \subseteq \mathcal{N}\setminus \mathcal{N}_{\mu}$ be the set of neighboring nodes to which microgrid ${\mu}$ is connected. 
% Suppose Assumption \ref{as: y_matrix sign} holds for network $\mathcal{G}$.
% %
% Moreover, assume either network $\mathcal{G}$ is lossless or its reduced
% nodal admittance matrix with respect to subsets of passive nodes $\mathcal{N}_{\mu}\setminus\alpha$ satisfy Assumption \ref{as: y_matrix bound}.
% %
% After Kron reducing the passive nodes in microgrid $\mu$, a node $i\in\alpha$ is connected to a node $k\in\gamma$ if and only if there is a path from $i$ to $k$ in network $\mathcal{G}$ whose nodes all belong to  $(\mathcal{N}_{\mu} \setminus \alpha) \cup \{i,k\}$. 
% %
% %Kron reduced microgrid $\mathcal{G}_i^r$ is also connected to the nodes $\alpha$. 
% \end{proposition}

% Appendix \ref{sec: proof of prop: effects of Kron reduction}



